The VC Dimension of Metric Balls under Fr\'echet and Hausdorff Distances

The Vapnik-Chervonenkis dimension provides a notion of complexity for systems of sets. If the VC dimension is small, then knowing this can drastically simplify fundamental computational tasks such as classification, range counting, and density estimation through the use of sampling bounds. We analyze set systems where the ground set $X$ is a set of polygonal curves in $\mathbb{R}^d$ and the sets $\mathcal{R}$ are metric balls defined by curve similarity metrics, such as the Fr\'echet distance and the Hausdorff distance, as well as their discrete counterparts. We derive upper and lower bounds on the VC dimension that imply useful sampling bounds in the setting that the number of curves is large, but the complexity of the individual curves is small. Our upper bounds are either near-quadratic or near-linear in the complexity of the curves that define the ranges and they are logarithmic in the complexity of the curves that define the ground set.

==> extensions.tex <==
\section{The Fr\'echet distance in higher dimensions}

In this section we assume Euclidean spaces of higher dimension ($d>2$) as the ambient space of the curves of the ground set.  
Let $\WW_m^d$ be the set of polygonal curves of complexity $m$ in $\RR^d$; for each $s\in \WW_m^d$, we associate an ordered set of vertices $V(s)$ and an ordered set of edges $E(s)$. 
Here, we investigate the case of the continuous Fr\'{e}chet distance in higher dimensions.\footnote{We conjecture that, using the same techniques, similar results can be derived for the range space induced by the Hausdorff distance.}

\subsection{Our approach in higher dimensions}

We saw that our approach readily extends to higher dimensions in the discrete setting, where the ground set consists of (ordered) point sets. However, in order to extend our bounds to higher ambient dimensions in the continuous setting, where the ground set consists of continuous curves (resp., sets of line segments), we invoke a powerful theorem by Anthony and Bartlett. We emphasize that, while it might be possible to apply this theorem directly to the range space in question, this would lead to substantially higher upper bounds. In particular we would not obtain a logarithmic dependency on the parameter $m$, the complexity of the ground set.

\begin{theorem}[Theorem 8.4 \cite{AB99}]
\label{theorem:predicatevc}
Suppose $h$ is a function from $\RR^d \times \RR^n$ to $\{0,1\}$ and let 
\[ H=\{x \mapsto h(\alpha,x):~\alpha \in \RR^d\}
\]
be the class determined by $h$. Suppose that $h$ can be computed by an algorithm that takes as input the pair $(\alpha,x) \in \RR^d \times \RR^n$ and returns $h(\alpha,x)$ after no more than $t$ operations of the following types:
\begin{itemize}
    \item the arithmetic operations $+,-,\times,$ and $/$ on real numbers,
    \item jumps conditioned on $>, \geq,< , \leq ,=,$ and $\neq$ comparisons of real numbers, and 
    \item output $0$ or $1$.
\end{itemize}
Then, the VC dimension of $H$ is $\leq 4d(t+2)$.
\end{theorem}

\subsection{Representation in terms of predicates}
\label{subsection:predicateshighd}
We need to use high-dimensional analogues of the predicates $P_1-P_6$ from Section~\ref{SSwF}. Correctness follows from Lemma~\ref{lemma:lem9}. 

Regarding predicates $P_5,P_6$, Lemma \ref{lemma:lem16} allows us to focus on two predicates: $d \wedge e \wedge f $ and $l\equiv h\lor (d\wedge e \wedge i) $. Predicate ${d \wedge e}$ can be simulated by predicate $l$, since any ball can be considered as an intersection of two identical balls. 

\hl{For} predicates $P_3$, $P_4$ we introduce two new low-level predicates:
\footnote{notation}
\begin{itemize}
    \item [$(a)$] given a segment $\overline{q_iq_{i+1}}$ and a point $s_j$, if $\|q_i -s_j\|\leq r$ or $\|q_{i+1} -s_j\|\leq r$  then output true. Otherwise, output false.  
    \item [$(b)$] given a segment $\overline{q_iq_{i+1}}$ and a point $s_j$, determine whether $s_j\in h(q_i,q_{i+1}-q_i) \cap h(q_{i+1},q_{i}-q_{i+1})$, where $h(x,y)$ is a halfspace defined by point $x$, i.e.~$x\in h(x,y)$, and the direction given by the vector $y$.
\end{itemize}
\begin{lemma}
\label{lemma:hdpredicatesp3p4}
Given the truth values of the predicates $(a)$, $(b)$, $(l)$ one can determine the truth value of the predicate $P_3$ (resp. $P_4$).
\end{lemma}
\begin{proof}
\hl{explain more?}
Basically, predicate $(b)$ determines whether the distance between a point and a line or between two points, is relevant.
If  $s_j\in h(q_i,q_{i+1}-q_i) \cap h(q_{i+1},q_{i}-q_{i+1})$ (predicate $(b)$)  then we return the output of the predicate $(l)$. 
If  $s_j\notin h(q_i,q_{i+1}-q_i) \cap h(q_{i+1},q_{i}-q_{i+1})$ then output  $(\|s_j-q_i \|\leq r) \lor (\|s_j-q_{i+1} \|\leq r)$ (predicate $(a)$).
\end{proof}

To conclude, the predicates that are needed are $P_1$, $P_2$, $(a)$, $(b)$, $(f) $ and $(l)$.


\if 0
To that end, we focus on generalizing the predicate $l$ as defined in Section \ref{section:haus} to higher dimensions. In particular, we need a predicate of the form: 
given an edge $\overline{q_iq_{i+1}}$, and points $s_j$, $s_t$, determine whether $\ell(\overline{q_iq_{i+1}})\cap D_r^d(s_j)\cap D_r^d(s_t) \neq \emptyset$. 
\fi

\subsection{Representation as a range space}
The predicate $l$ naturally defines the following range space: let $ \RR^d\times \RR^d$ be the ground set, and let $\RRR=\bigcup_{r\geq0}\{R_{\overline{q_i q_{i+1}}}^r\mid \overline{{q_i q_{i+1}}} \in \WW_2^d \}$, where 
\[R_{\overline{q_i q_{i+1}}}^r=\{(x,y) \mid x,y\in \RR^d, \ell(\overline{q_iq_{i+1}})\cap D_r^d(x)\cap D_r^d(y) \neq \emptyset\},\] be the range set. The second range space of interest is the dual of the above: let $\WW_2^d$ be the ground set of line segments and let $\RRR=\bigcup_{r\geq 0}\{R_{s_i,s_j}^r \mid s_i,s_j \in \RR^d\}$ , where 
\[R_{s_is_j}^r=\{\overline{xy} \mid \overline{xy} \in \WW_2^d,\ell(\overline{xy})\cap D_r^d(s_j)\cap D_r^d(s_i) \neq \emptyset \}.\] The VC dimension of both range spaces can be bounded by making use of theorem~\ref{theorem:predicatevc} by Anthony and Bartlett. 


\begin{theorem}
\label{theorem:lpredicate}
Let $h$ be a function implementing predicate $(l)$: given $r>0$,  a line $\ell$ and two points $x,y \in \RR^d$, it outputs $1$ when $\ell \cap D_r^d(x) \cap D_r^d(y) \neq \emptyset$, and it outputs $0$ otherwise. The function $h$ can be implemented by making use of $O(d)$ operations of the following types:
\begin{itemize}
    \item the arithmetic operations $+,-,\times,$ and $/$ on real numbers,
    \item jumps conditioned on $>, \geq,< , \leq ,=,$ and $\neq$ comparisons of real numbers, and 
    \item output $0$ or $1$.
\end{itemize}

\end{theorem}
\begin{proof}
The input line is defined by an equation $\ell(t)=u+tv$, where $u=(u_1,\ldots,u_d)\in \RR^d$, $v=(v_1,\ldots,v_d)\in\RR^d$ and $t\in \RR$. The two balls are defined by equations of the form $\|x-p\|^2 \leq r^2$ and $\|x-q\|^2 \leq r^2$, where $x\in \RR^d$, $p=(p_1,\ldots,p_d)\in \RR^d$, $q=(q_1,\ldots, q_d) \in \RR^d$ are the two centers of the two balls and $r>0$. We now make use of the standard parabolic lifting of points $(x_1,\ldots,x_d) \mapsto \left(x_1,\ldots,x_d, \sum_{i=1}^d x_i^2 \right)$. Hence, the lifted objects are defined as follows:
\begin{itemize}
    \item $\ell'(t)=\left( u_1+t v_1,\ldots, u_d+tv_d, \sum_{i=1}^d (u_i+tv_i)^2\right),$
    \item $a(x)\leq 0$, where $a(x)=\sum_{i=1}^{d+1} a_i x_i' -a_0   $, $a_0 = r^2-\sum_{i=1}^d p_i$, for $i=1,\ldots,d$: $a_i=-2p_i$, $a_{d+1}=1$, for $i=1,\ldots,d$: $x_i'=x_i$, and $x_{d+1}'=\sum_{i=1}^d x_i^2$,
    \item $b(x)\leq 0$, where $b(x)=\sum_{i=1}^{d+1} b_i x_i' -b_0  \leq 0  $, $b_0 = r^2-\sum_{i=1}^d q_i$, for $i=1,\ldots,d$: $b_i=-2q_i$, $b_{d+1}=1$, for $i=1,\ldots,d$: $x_i'=x_i$, and $x_{d+1}'=\sum_{i=1}^d x_i^2$,
\end{itemize}
and they have a non-empty intersection if and only if the input line and the two balls have a non-empty intersection.

Now the intersection between these three, is defined by the two inequalities $a(\ell(t))\leq 0$, $b(\ell(t))\leq 0$. Notice that the leading coefficient of both polynomials $a(\ell(t)),b(\ell(t))$ is $\sum_{i=1} v_i^2$ and hence both are convex. This implies that $\exists t ~a(\ell(t))\leq 0, b(\ell(t))\leq 0  \implies \exists t~ a(\ell(t))=b(\ell(t)) \text{ and } a(\ell(t)))\leq 0$. Furthermore, the direction $\exists t~ a(\ell(t))=b(\ell(t)) \text{ and } a(\ell(t)))\leq 0 \implies \exists t ~a(\ell(t))\leq 0, b(\ell(t))\leq 0$ is trivial. Hence, it suffices to determine whether there exists a $t^o \in \RR$ s.t.~$a(\ell(t^o))-b(\ell(t^o))=0$ and $a(\ell(t^o))\leq 0$. 

Now, notice that the term which is quadratic in $t$ vanishes:  
\[ a(\ell(t)) - b(\ell(t))=\sum_{i=1}^d a_i (u_i+tv_i)-a_0 -\sum_{i=1}^d b_i (u_i+tv_i)-b_0.  
\]
Hence, we are able to solve for $t$, and then evaluate the quadratic polynomial $a(\ell(t))$. The number of arithmetic operations of the types which are described above, are bounded by $O(d)$. 
\end{proof}
Now, consider any two polygonal curves $s$ and $q$  with vertices $s_1,\ldots,s_m$ and $q_1,\ldots,q_k$ respectively. 
In addition to the high dimensional analogues of $P_1^r(q,s),P_2^r(q,s)$ which were defined in Section~\ref{SSwF:sets}, we need to define sets which correspond to predicates $P_3,P_4,P_5,P_6$. Some of these sets are just high-dimensional analogues of the sets which were defined in Subsection \ref{subsection:predicateshighd}. We \hl{define} the sets \footnote{maybe change notation for general d?}
 \begin{itemize}
  \item $P_1^r(q,s)=D_r^d (q_1) \cap V(s) $,
  \item $P_2^r(q,s)=D_r^d (q_k) \cap V(s)$,
 \item $P_{a}^r(q,s)= \{D_r^d (q_i)\cap V(s) \mid q_i \in V(q)\} $,
  \item $P_{a}^{ r \prime} (q,s)= \{D_r^d (s_i)\cap V(q) \mid s_i \in V(s)\}$ , 
  \item $P_{b}^r(q,s)= \{h(q_i,q_{i+1}-q_i) \cap h(q_{i+1},q_{i}-q_{i+1})\cap V(s) \mid \overline{q_i q_{i+1}}\in E(q)\}$, where $h(x,y)$ is a halfspace \hl{defined by} point $x$, and the direction given by the vector $y$,
\item $P_{b}^{r \prime} (q,s)=\{h(s_i,s_{i+1}-s_i) \cap h(s_{i+1},s_{i}-s_{i+1})\cap V(q)\mid \overline{s_{i+1}s_i}\in E(s)\}$, where $h(x,y)$ is a halfspace \hl{defined by} point $x$,  and the direction given by the vector $y$,
\item $P_{f}(q,s)=\{ \{x\in \RR^d\mid \langle q_{i+1}-q_i,x \rangle \geq 0\} \cap \tilde{V}(s)   \}$, where $\tilde{V}(s)=\{s_k-s_j \mid k>j,~s_k,s_j\in V(s) \}$,
\item $P_{f}'(q,s)=\{ \{x\in \RR^d\mid \langle s_{i+1}-s_i,x \rangle \geq 0\} \cap \tilde{V}(q)   \}$, where $\tilde{V}(q)=\{q_k-q_j \mid k>j,~q_k,q_j\in V(q) \}$,
\item $P_l^r(q,s)=\{R_{\overline{q_i q_{i+1}}}^r \cap (V(s) \times V(s)) \mid   \overline{q_i q_{i+1}}\in E(q)\}$,
\item $P_l^{r\prime}(q,s)=\{R_{s_i,s_j}^r \cap E(q) \mid   s_i ,s_j\in V(s)\}$.
 \end{itemize}

\begin{lemma}
\label{lemma:cfsetshd}
Let $s$ be a polygonal curve in $\WW_m^d$ with vertices $s_1,\ldots,s_m$ and $q$ be a polygonal curve in $\WW_k^d$ with vertices $q_1,\ldots,q_k$. Fix any $r\geq 0$.  
The following sets are sufficient in order to determine whether $\d_F(s,q)\leq r$ 
or $\d_F(s,q)> r$:
\begin{align*}
    & P_1^r(q,s),P_2^r(q,s),P_{a}^r(q,s),P_{a}^{r \prime}(q,s),P_{b}^r(q,s),P_{b}^{r\prime}(q,s) ,P_{f}(q,s),P_{f}'(q,s),P_{l}^r(q,s),
     P_{l}^{r \prime}(q,s).
\end{align*}
\end{lemma}

\begin{proof}
\hl{maybe explain more?}
Sets $P_1^r(q,s),P_2^r(q,s)$ uniquely define the output of predicates $P_1,P_2$. Then, sets $P_{a}^r(q,s),P_{a}^{r \prime}(q,s),P_{b}^r(q,s),P_{b}^{r \prime}(q,s)$ uniquely define the output of predicates $(a)$, $(b)$, and by Lemma \ref{lemma:hdpredicatesp3p4}, they also define the output of $P_3$, $P_4$. 
%In particular, predicate $(a)$ corresponds to $\left[s_j\in D_r^d(q_i)\right]\lor \left[s_j\in D_r^d(q_{i+1})\right]$
Finally, $P_{f}(q,s),P_{f}'(q,s),P_{l}^r(q,s),P_{l}^{r,\prime}(q,s)$ uniquely define the output of $(f)$ and $(l)$ and as a consequence they also define the output of $P_5$, $P_6$, due to Lemma \ref{lemma:lem16}.
\end{proof}


\subsection{VC dimension bounds}
The sets which are used in Lemma \ref{lemma:cfsetshd} define simple range spaces e.g.~primal and dual range spaces induced by halfspaces or balls and range spaces which are induced by predicates as in Theorem \ref{theorem:lpredicate}. The former range spaces are known to have bounded VC dimension (see e.g.\cite{2017handbook}) of $O(d)$, while the latter can be bounded by Theorem \ref{theorem:predicatevc}. 



\begin{theorem}
\label{TFr}
Let $\RRR_{F}$ be the set of all \nnms, under the  
Fr\'{e}chet distance, centered at polygonal curves in $\WW_k^d$. The VC dimension of 
$(\WW_m^d,\RRR_{F})$ is ${O}\left(d^2 k^2 \log (km)\right)$.
\end{theorem}
\begin{proof}

Let $S\subset \WW_m^d$ be a set of $t$ polygonal curves and let $q\in \WW_k^d$. By Lemma \ref{lemma:cfsetshd}, the set $\{s\in S \mid d_F(s,q)\leq r\}$ is uniquely defined by the sets 
\[
     \bigcup_{s\in S} P_1^r(q,s),\bigcup_{s\in S} P_2^r(q,s), \bigcup_{s\in S} P_{a}^r(q,s),\bigcup_{s\in S} P_{a}^{r \prime}(q,s),\bigcup_{s\in S} P_{b}^{r }(q,s),\bigcup_{s\in S} P_{b}^{r \prime }(q,s) ,\bigcup_{s\in S} P_{f}(q,s), \]
    \[\bigcup_{s\in S} P_{f}'(q,s),\bigcup_{s\in S} P_{l}^r(q,s),
     \bigcup_{s\in S} P_{l}^{r \prime}(q,s).
\]
The range spaces which correspond to sets $\bigcup_{r\geq0}\bigcup_{s\in S} P_1^r(q,s)$, $\bigcup_{r\geq0} \bigcup_{s\in S} P_2^r(q,s)$, $\bigcup_{r\geq0} \bigcup_{s\in S} P_{a}^r(q,s)$, $\bigcup_{r\geq0} \bigcup_{s\in S} P_{a}^{r \prime}(q,s)$ are the primal and dual range spaces induced by balls. Hence, there are at most $(tm)^{O(d)}$ such sets.  

Then, $\bigcup_{r\geq0} \bigcup_{r\geq0}\bigcup_{s\in S} P_{b}^r(q,s)$ corresponds to the range space, where the ground set consists of $tm$ points and the ranges are defined as an intersection of two halfspaces. Hence, there are at most $(tm)^{O(d)}$ such sets. The set $\bigcup_{r\geq0}\bigcup_{s\in S} P_{b}^{r \prime}(q,s)$ corresponds to the dual range space. Notice, that the ground set now consists of $tm$ intersections of halfspaces, and there are $2tm$ different halfspaces. The  halfspace-halfspace intersections which are stabbed by points are uniquely defined by the halfspaces which are stabbed by points. Hence, by the VC dimension bounds of the dual space induced by halfspaces, we obtain an upper bound of $(tm)^{O(d)}$ on the number of different sets $\bigcup_{r\geq0} \bigcup_{s\in S} P_{b}^{r \prime}(q,s)$,

The sets $\bigcup_{s\in S} P_{f}(q,s)$, $\bigcup_{s\in S} P_{f}'(q,s)$ corresponds to the primal and dual range spaces induced by halfspaces, which implies an upper bound of $(tm)^{O(d)}$ on the number of different such sets. 

Finally, in order to bound the shattering dimension of the range spaces induced by 
$\bigcup_{r\geq0}\bigcup_{s\in S} P_{l}^r(q,s)$, $\bigcup_{r\geq0}\bigcup_{s\in S} P_{l}^{r \prime}(q,s)$, we invoke Theorems \ref{theorem:predicatevc}, \ref{theorem:lpredicate}, which imply an upper bound of $(tm)^{O(d^2)}$.
\end{proof}

